Tutorial on the Executable ASM Specification of the AB Protocol and Comparison with TLA$^+$

The main aim of this report is to provide an introductory tutorial on the Abstract State Machines (ASM) specification method for software engineering to an audience already familiar with the Temporal Logic of Actions (TLA$^+$) method. The report asks to what extent the ASM and TLA$^+$ methods are complementary in checking specifications against stated requirements and proposes some answers. A second aim is to provide a comparison between different executable frameworks that have been developed for the same specification languages. Thus, the ASM discussion is complemented by executable Corinthian ASM (CASM) and CoreASM models. Similarly, the two TLA$^+$ specifications presented, which rely on the TLC and Apalache model checkers, respectively, are complemented by a Quint specification, a new language developed by Informal Systems to serve as a user-friendly syntax layer for TLA$^+$. For the basis of comparison we use the specification of the Alternating Bit (AB) protocol because it is a simple and well-understood protocol already extensively analysed in the literature. While the models reported here and developed with the two methods are semantically equivalent, ASMs and Quint are better suited for top-down specification from abstract requirements by iterative refinement. TLA$^+$ seems to be more easily used bottom-up, to build abstractions on top of verified components in spite of the fact that it, too, emphasizes iterative refinement. In the final section, the report begins to scope out the possibility of a homomorphism between the specification of the AB protocol and its finite-state machine (FSM) through state space visualizations, motivated by a search for a formal decomposition method.

==> ArXiv Submission 2/Misc/lst-coream-conf.tex <==
\usepackage{listings}
\usepackage{lstautogobble}

\renewcommand*\lstlistingname{Specification}
\renewcommand\lstlistlistingname{Specifications}
\providecommand*{\lstlistingautorefname}{spec.}
\providecommand*{\lstnumberautorefname}{line}

\lstset{numberbychapter=false}
\lstset{xleftmargin=0.66cm} %line numbers take some additional place
\lstset{xrightmargin=0.18cm} %no linenumbers used
\lstset{captionpos=b}
\lstset{numbers=left}
\lstset{basicstyle=\small\ttfamily}
\lstset{numberstyle=\tiny\ttfamily}
\lstset{tabsize=4}
%\lstset{showstringspaces=true}

\makeatletter
\newcounter{asmcounter}[section]
\renewcommand{\theasmcounter}{\arabic{asmcounter}} 

\lstnewenvironment{lstasm}[2][]{
	\renewcommand*\lstlistingname{Specification}
	\renewcommand\lstlistlistingname{Specs.}
	\renewcommand*{\lstlistingautorefname}{spec.}
	\renewcommand*{\lstnumberautorefname}{line}
	\let\c@lstlisting=\c@asmcounter
	\let\thelstlisting=\theasmcounter
	\lstset{language=ASM, #1}
} {}

\newcommand\includelst[1][]{
	\renewcommand*\lstlistingname{Specification}
	\renewcommand\lstlistlistingname{specs.}
	\renewcommand*{\lstlistingautorefname}{spec.}
	\renewcommand*{\lstnumberautorefname}{line}
	\let\c@lstlisting=\c@asmcounter
	\let\thelstlisting=\theasmcounter
	\expandafter\lstinputlisting\expandafter[language=ASM, #1]
}
\makeatother

% % % Code-Formatierungen & Farben % % %
\definecolor{lightlightgray}{gray}{0.9}
%http://colorschemedesigner.com/#0941Qqau-w0w0
\definecolor{primary}{HTML}{F7542D} %orange
\definecolor{secondary}{HTML}{F7932D} %brown
\definecolor{tertiary}{HTML}{207F9A} %blue
\definecolor{fourth}{HTML}{008000} %green
\definecolor{fifth}{HTML}{800000} %red

%Formatierung von Schlüsselwörtern und/oder stehenden Begriffen
\newcommand{\aspectj}[1]{\textit{#1}}
\newcommand{\aoasm}[1]{\textsf{#1}}
\newcommand{\java}[1]{\textemdash{#1}}
\newcommand{\uml}[1]{\textsl{#1}}

\newcommand{\coreasm}[1]{\lstinline[mathescape]|#1|}
%can only be used within math environment or \asm command content
\newcommand{\asmtag}[1]{\flq$#1$\frq}

\newcommand{\asmlstkeyword}{\color{fifth}\bfseries}
\newcommand{\asmlstrule}{\ttfamily}
\newcommand{\asmlstdomain}{\scshape\normalsize}
\newcommand{\asmlstfunction}{\rmfamily}
\newcommand{\asmlstpredicate}{\asmlstfunction \itshape}
\newcommand{\asmlstderived}{\asmlstfunction \slshape}
\newcommand{\asmlstvariable}{\ttfamily}
\newcommand{\asmlstconstant}{\em}
\newcommand{\asmstring}{\color{fourth}\ttfamily}
\newcommand{\asmlstcommentstyle}{\rmfamily\color{gray}}

%removes tree whitespaces at the beginning of each line
%useful for includes from files
\lstset{autogobble=true}

\lstset{
	aboveskip=1.2em,
	belowskip=1.2em,
	framexleftmargin=5pt,
	columns=fullflexible, keepspaces, %if non monospaced font is choosen, preserve whitespaces after replaced literals
	frame=b,
	inputencoding={utf8}, extendedchars=false,
%	basicstyle=\small\rmfamily,
	literate=%
    {,}{{$,$}}1
    {.}{{$.$}}1
    {[}{{$[$}}1
    {]}{{$]$}}1
    {|}{{$|$}}1
    {-}{{$-$}}1
    {+}{{$+$}}1
    {*}{{$*$}}1
    {=}{{$=$}}1
    {:=}{{$\:=$}}1
    {:}{{$:$}}1
    {!=}{{$\neq$}}1
    {>}{{$>$}}1
    {<}{{$<$}}1
    {<=}{{$\leq$}}1
    {>=}{{$\geq$}}1
    {<>}{{$\neq$}}1
    {(|}{{$(\hspace{0.09em}\mathllap{|}$}}1
    {|)}{{$\mathrlap{|}\hspace{0.09em})$}}1
    {\{|}{{$\{\hspace{0.07em}\mathllap{|}$}}1
    {|\}}{{$\mathrlap{|}\hspace{0.07em}\}$}}1
    {[[}{{$[\hspace{0.09em}\mathllap{[}$}}1
    %{[[}{{$\textlbrackdbl$}}1
    {]]}{{$\mathrlap{]}\hspace{0.09em}]$}}1
    %{]]}{{$\textrbrackdbl$}}1
    {<-}{{$\leftarrow$}}1
    {->}{{$\rightarrow$}}1
    {times}{{$\times$}}1
    {<<}{{\texttt{\flqq}}}1
    {<}{{\texttt{\flq}}}1
    {>>}{{\texttt{\frqq}}}1
    {>}{{\texttt{\frq}}}1
    %{memberof}{{$\in$}}1
    ,
	 commentstyle=\asmlstcommentstyle,
	 sensitive=true,
	 morecomment=[s]{/*}{*/},
	 morecomment=[is]{/i}{ i/}, %invisible comment
	 morecomment=[l]{//},
	 escapeinside={/@}{@/},
	 stringstyle=\asmstring,
	 showstringspaces=false,
	 morestring=[b]"",
	 morestring=[b]",
	 backgroundcolor=\color{white},
	 mathescape=true,
	 breaklines=true,
	 breakatwhitespace=true,
	 linewidth=\textwidth,
	 frame=l,
	 float=ht,
	 numbers=none,
	 numberstyle=\tiny,   % Stil der Zeilennummern
	 numbersep=10pt,    % Abstand der Nummern zum Text
	 captionpos=b,
	 tabsize=3,
	 tab=\smash{\rule[-.2\baselineskip]{.4pt}{\baselineskip}\kern.5em},
	 keywordstyle=[1]{\asmlstkeyword}, % ASM keywords - lowercase
	 morekeywords=[1]{
	 abstract, rule, enum, function, derived, local, shared, universe, call, case, choose, CoreASM, CoreModule, of, if, ifnone, implies, import, then, else, with, exists, extend, include, remove, from, add, to, seq, memberof, next, iterate, skip, forall, in, do, enditerate, endchoose, endcase, endforall, endif, is, return, result, print, before, around, after, undef, true, false, initially, resume, init, option, suspend, and, or, not, pick, par, endpar,self, seqblock, endseq, endseqblock, let, holds, use, @, ?, :, xor,while, shift, left, right, into, enqueue, dequeue, push, pop
	 }, 
	 keywordstyle=[2]{\asmlstrule}, %ASM rules - upper case camel cased
	 morekeywords=[2]{
	 }, 
	 keywordstyle=[3]{\asmlstdomain}, %ASM domains - upercase camel cased
	 morekeywords=[3]{
	 	Agents, Number, Number_Range, Boolean, Element, String, Function, Set, List, Map
	 },
	 keywordstyle=[4]{\asmlstpredicate},%PREDICATES - upper came cased
	 morekeywords=[4]{
	 },
	 keywordstyle=[5]{\asmlstfunction}, %FUNCTIONS - lower camel cased
	 morekeywords=[5]{
		program
	 },
	 keywordstyle=[6]{\asmlstderived}, %DERIVED FUNCTIONS - lower camel cased
	 morekeywords=[6]{
	 subset, union, intersect, diff
	 },
	 keywordstyle=[7]{\asmlstvariable}, %VARIABLES lower camel cased
	 morekeywords=[7]{
	 },
	 keywordstyle=[8]{\asmlstconstant}, %CONSTATNTS VALUES / ENUM VALUES lower camel cased
	 morekeywords=[8]{
	 id, loc, value, guard, function, bin-op, expression, filename
	 }
}
\newcommand{\AsmKeyword}[1]{\lstset{morekeywords=[1]{#1}}}
\newcommand{\AsmRule}[1]{\lstset{morekeywords=[2]{#1}}}
\newcommand{\AsmDomain}[1]{\lstset{morekeywords=[3]{#1}}}
\newcommand{\AsmPredicate}[1]{\lstset{morekeywords=[4]{#1}}}
\newcommand{\AsmFunction}[1]{\lstset{morekeywords=[5]{#1}}}
\newcommand{\AsmDerivedFunction}[1]{\lstset{morekeywords=[6]{#1}}}
\newcommand{\AsmVariable}[1]{\lstset{morekeywords=[7]{#1}}}
\newcommand{\AsmConstantOrEnum}[1]{\lstset{morekeywords=[8]{#1}}}

\newcommand{\asmboxed}[1]{\fontsize{7}{8.4}\ensuremath{\boxed{\hspace{-.175em}#1\hspace{-.175em}}}}

==> ArXiv Submission 2/Misc/macros.tex <==
%------------------------------------------------------------------------
% TeX and LaTeX macros
%------------------------------------------------------------------------
%
% In math formulas we use italic instead of mathitalic
%
\makeatletter
% ~ gives a \; space in math mode
\def~{\ifmmode\;\else\penalty\@M\ \fi}
%  Italic in mathematical formulas
\def\@setmcodes#1#2#3{{\count0=#1 \count1=#3
  \loop \global\mathcode\count0=\count1 \ifnum \count0<#2
  \advance\count0 by1 \advance\count1 by1 \repeat}}
\DeclareSymbolFont{italic}{OT1}{\rmdefault}{m}{it}
\let\mathit\undefined
\DeclareSymbolFontAlphabet{\mathit}{italic}
\edef\@tempa{\hexnumber@\symitalic}
\@setmcodes{`A}{`Z}{"7\@tempa41}
\@setmcodes{`a}{`z}{"7\@tempa61}
\makeatother
%
% \begin{asm} ... \end{asm}
%
\newdimen\asmindent     
\asmindent=\parindent
\newcount\asmi
\def\inc{\global\advance\asmi by 1}
\def\dec{\global\advance\asmi by-1}
\def\nl{{}$\par\hangindent\asmi em
  \noindent\kern\asmi em\ignorespaces$} 
\def\asmskip{{}$\par\smallskip\hangindent\asmi em
  \noindent\kern\asmi em\ignorespaces$} 
\def\asm{\global\asmi=0 
%%%%%%%%%%%%%% added by Paolo:
\parskip=0pt
%%%%%%%%%%%%%%%%%%%%%%%
 \def\+{\inc\nl}
 \def\-{\dec\nl}
 \def\\{\nl}
 \begin{trivlist}\item[]\leftskip=\asmindent\relax$}
\def\endasm{$\end{trivlist}}
%\mathindent=\asmindent
%
% \begin{asmarray}
%    f(s_1) & := t_1 \\
%    f(s_2) & := t_2 
% \end{asmarray}
%
\def\asmarray{\begin{array}[t]{@{}l@{\;}l@{\;}l@{}}}
\def\endasmarray{\end{array}}
%
%
%
\def\asmcomment#1{\quad\hbox{// #1}}
%
%  \begin{subasm} ... \end{subasm}
%
\newcount\asmii
\def\subasm{\vtop\bgroup\asmii=0\normalbaselines
 \def\nl##1{$\egroup\advance\asmii by##1\relax\hbox\bgroup\hskip\asmii em$}
 \def\\{\nl{0}}
 \def\+{\nl{1}}
 \def\-{\nl{-1}}
 \hbox\bgroup\hskip\asmii em$}
\def\endsubasm{$\egroup\egroup}
%
% Keywords in ASM code
%
\def\ASM#1{\hbox{\sc#1}}        % rule names and macros
\def\ASMIND#1{\ASM{#1}\index{#1@{\sc#1}}}
\def\AWAIT   {\mathrel{\mathbf{await}}}
\def\AND     {\mathrel{\mathbf{and}}}
\def\CASE    {\mathrel{\mathbf{case}}}
\def\CHOOSE  {\mathrel{\mathbf{choose}}}
\def\CREATE  {\mathrel{\mathbf{create}}}
\def\NEW  {\mathrel{\mathbf{new}}}
\def\DO      {\mathrel{\mathbf{do}}}
\def\ELSE    {\mathrel{\mathbf{else}}}
\def\ELSEIF  {\mathrel{\mathbf{elseif}}}
\def\FORALL  {\mathrel{\mathbf{forall}}}
\def\FORSOME  {\mathrel{\mathbf{forsome}}}
\def\FOREACH  {\mathrel{\mathbf{foreach}}}
\def\FROM  {\mathrel{\mathbf{from}}}
\def\THEREISNO  {\mathrel{\mathbf{thereisno}}}
\def\IF      {\mathrel{\mathbf{if}}}
\def\IFF      {\mathrel{\mathbf{iff}}}
\def\IMPORT  {\mathrel{\mathbf{import}}}
\def\IN      {\mathrel{\mathbf{in}}}
\def\LET     {\mathrel{\mathbf{let}}}
\def\SELF    {\mathrel{\mathbf{self}}}
\def\MATCH    {\mathrel{\textbf{match}}}
\def\NOT     {\mathrel{\mathbf{not}}}
\def\OF      {\mathrel{\mathbf{of}}}
\def\OR      {\mathrel{\mathbf{or}}}
\def\PAR     {\mathrel{\mathbf{par}}}
\def\SEQ     {\mathrel{\mathbf{seq}}}
\def\SKIP    {\mathrel{\mathbf{skip}}}
\def\THEN    {\mathrel{\mathbf{then}}}
\def\TO  {\mathrel{\mathbf{to}}}
\def\WHERE   {\mathrel{\mathbf{where}}}
\def\WHILE   {\mathrel{\mathbf{while}}}
\def\UNDEF   {\mathrel{\mathbf{undef}}}
\def\UNTIL   {\mathrel{\mathbf{until}}}
\def\WHEN   {\mathrel{\mathbf{when}}}
\def\WITH    {\mathrel{\mathbf{with}}}
\def\STEP    {\mathrel{\mathbf{step}}}
\def\STEPWISE    {\mathrel{\mathbf{stepwise}}}
\def\SEQ    {\mathrel{\mathbf{seq}}}
\def\RESULT  {\mathrel{\mathbf{result}}}
\def\CALL  {\mathrel{\mathbf{Call}}}
\def\LOCAL    {\mathrel{\mathbf{local}}}
\def\ADDGUARD {\mathrel{\mathbf{addGuard}}}
\def\ADDUPD   {\mathrel{\mathbf{addUpd}}}
\def\ADDRULE  {\mathrel{\mathbf{addRule}}}
\def\MINUSRULE  {\mathrel{\mathbf{minusRule}}}
\def\TO      {\mathrel{\mathbf{to}}}
%
% Including figures
%
\def\includefig#1#2{\centering\medskip
  \includegraphics[scale=#1]{fig/#2}
  \medskip}
%
% References to paragraphs in the ECMA standard for C#
%
\def\ecma#1{\cite[\S#1]{ecma334}}
%
%  Environments for definitions and theorems
%
%\theorembodyfont{\rm}
%\newtheorem{definition}[subsection]{Definition}
%\newtheorem{lemma}[subsection]{Lemma}
%\newtheorem{theorem}[subsection]{Theorem}
%\newtheorem{proposition}[subsection]{Proposition}
%\newtheorem{corollary}[subsection]{Corollary}
%\newtheorem{example}[subsection]{Example}
%\newtheorem{remark}[subsection]{Remark}
%\newtheorem{constraint}[subsection]{Constraint}
\def\proof{\trivlist\item[]{\bf Proof.}}
\def\endproof{$\Box$\endtrivlist}
%
% enumerate and itemize (smaller skips) from "latex.ltx"
%
\makeatletter
\def\enumerate{%
  \ifnum \@enumdepth >\thr@@\@toodeep\else
    \advance\@enumdepth\@ne
    \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
      \expandafter
      \list
        \csname label\@enumctr\endcsname
        {\usecounter\@enumctr\def\makelabel##1{\hss\llap{##1}}
         \itemsep 0pt\parskip 0pt\parsep 0pt\topsep\smallskipamount}%
  \fi}
\def\itemize{%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
    \advance\@itemdepth\@ne
    \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
    \expandafter
    \list
      \csname\@itemitem\endcsname
      {\def\makelabel##1{\hss\llap{##1}}
       \itemsep 0pt\parskip 0pt\parsep 0pt\topsep\smallskipamount}%
  \fi}
\makeatother
%
% items in itemize
%
\def\bull{\vrule height .9ex width .8ex depth -.1ex}
\def\labelitemi{\bull}
%
%
%
\def\cs#1{C\#$_{\mathcal{#1}}$}
\def\lang#1{L$_{\mathcal{#1}}$}
%
% Positions
%
\def\pos#1{{}^{#1}}
\def\termPos{\blacktriangleright}
\def\cursor{\pos{\termPos}}
%
%
%
\def\sup{\hbox{sup}}
\def\c#1{\texttt{#1}}           % code
\def\N#1{\textit{#1}}           % non terminal symbols
\def\T#1{\hbox{`\texttt{#1}'}}  % terminal symbols
\def\A#1{\hbox{\sc#1}}          % ASM rules
\def\D#1{#1}                    % dynamic functions
\def\U#1{#1}                    % universes
\def\C#1{#1}                    % constructors
\def\rdef{\equiv}
\def\lbr{\c{\char`\{}}
\def\rbr{\c{\char`\}}}
\def\mb{\hbox{::}}
\def\map#1#2{\textbf{Map from}~#1~\textbf{to}~#2}
\def\cat{\cdot}
\def\adots{\mathinner{\ldotp\ldotp}}
%
%
% macros.tex ends here
